Chemical abundances in 7 metal-poor HII regions and a determination of the primordial helium abundance

We conducted a long-slit spectrophotometry analysis to obtain the chemical abundances of seven metal-poor HII regions in three galaxies: UM 160, UM 420, and TOL 0513-393. The data have been taken with the Focal Reducer Low Dispersion Spectrograph 1 (FORS1) at the 8.2-m Very Large Telescope. We derived the physical conditions and the chemical abundances of N, O, Ne, S, Ar, and Cl. We also performed a detailed analysis that involves abundance determinations using the $t^2$ formalism. Based on HeI recombination line intensity ratios, together with the Helio14 code, we derived the abundance of He. In addition, for a value $\Delta Y/\Delta Z_O =3.3\pm 0.7$, we have estimated that the primordial helium abundance by mass is $Y_{\rm P}=0.2448\pm0.0033$. This value agrees with values derived from Standard Big Bang Nucleosynthesis and with other recent determinations of $Y_{\rm P}$.

==> 7 HII regions - MNRS/referee.tex <==
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 

MAYO 24

Comments to the Author
I want to thank the authors for doing such a thorough job on their resubmission, and for returning the manuscript so promptly - I do not require to see another version of the manuscript. I've re-read through the paper and have a few final minor thoughts, but none of these affect the acceptance of their nice paper - thanks, and congratulations!

R:
y  versus  Y:
I'm not going to force this issue, but I raise it only to clarify what I discussed in my previous response, and the fact that the choice of "Delta Y / Delta Z_O" is the leading systematic uncertainty. In Table 6 the authors quote number abundances of He/H (so these do not depend on Delta Y / Delta Z_O). To mitigate this systematic, one could fit to the number abundances and derive a primordial number abundance by fitting a linear function to y versus O/H. The intercept would be y_p, which doesn't depend on the above-mentioned systematic. If you want to report Y_p, you could convert y_p into Y_p, and so you could eliminate one of your dominant systematics - I think!

A: 
As We understand this touches 2 different points: 
1st the choice of using y or Y 
--- both should give the same result for each object, and doing it by mass is much more common.
2nd looking for a fit using our data instead of the fit  we used in previous works.
--- any fit will have some uncertainty, but we have only a handful of points and they have a very large dispersion and not a wide enough baseline (in O/H) to provide us with better error bars.  

R:
Figure 2, spectroscopy inset:
In my comments on the previous version of the manuscript, I suggested putting 4 horizontal red lines on the spectroscopy (bottom right) panel. The authors mentioned that this was "Done", but the figure wasn't changed. While the figure doesn't need to be changed, I thought I would raise this, just in case the authors have an updated version of the figure that wasn't included in the submission.

A:
We have updated the figure.

R:
Section 6, paragraph starting with "In Table 7, we show...":
There is a typo in the text: "fist" --> "first"

A: 
Done

R:
Section 6, paragraph starting with "In Figure 4, we show...":
There is a typo in the text: "mater" --> "matter"

A:
Done

R:
Table 8 and Conclusions:
The authors mention "Delta Y / Delta O" in the caption of Table 8 and in the conclusions, and they may wish to correct this to read "Delta Y / Delta Z_O", to maintain consistency throughout the paper.

A: Done

R:
Conclusions, paragraph 3:
The references have not been updated in this paragraph.

A:
Done



% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 


MAYO 12

Reviewer's Comments:

R:
Comments to the Author
The authors present a nice paper about several H II regions in three nearby metal-poor galaxies. The main goal of the paper is to measure the chemical abundances and provide a new determination of the primordial helium abundance. The paper contains new high quality data, and I am happy to accept the manuscript for publication after the authors address a few comments that I have listed below.

-------

Main comments:
R:
1. Throughout the paper, the authors have listed all recent helium abundance determinations from H II regions, with the exception of one paper by Hsyu et al.
https://ui.adsabs.harvard.edu/abs/2020ApJ...896...77H/abstract
For completeness, the authors should probably include this determination of Yp in their work. It doesn't affect their results, and also shows a "below CMB" value of the primordial helium abundance.

A:
Sorry it was an oversight; it should have been mentioned several times throughout the paper. We now have included the reference in the introduction, Table 8, Figure 4, as well two times in section 6.

R:
2. Section 3 paragraph 2
"fitting the flux ratios of the brightest Balmer lines as compared with the theoretical values..."
Doesn't this require a temperature? If so, how does this affect the primordial helium abundance determination? Is this uncertainty included in the systematics budget?

A:
We have added a sentence after equation 1 to indicate that the HI lines have a small dependence on temperature, and that we need to do this process iteratively before being able to deredden the observed lines.

An uncertainty on the proper temperature when fitting the Balmer lines produces a very small difference on the final values, and it is indeed included in the error budget. A 500 degree error on the temperature of the fitting of the H I lines will produce a very small difference in the line intensities, and the overall effect will be an error similar or smaller than 0.0001 on YP. (Of course the temperature dependence on the final determination propagates into other aspects of the final determination; but we believe we have also carefully considered and included them on the final budget: the overall ratio of HeI/HI emmisivities, the O abundance and Delta Y / Delta Z_O correction, the collisional excitation of the H and He lines)

R:
3. Table 2
Two comments: The authors quote a percentage error of each line intensity. Does this include the uncertainty of the flux calibration based on the standard star? Going further, is the error reported just the statistical error, or does it include other terms? It's best to mention this explicitly in the text.

A:
We now include this information on the last paragraph of section 3.

R:
4. Table 2
I wonder if this table would be better suited to a Supplementary table online? On the final page of the Table, there are three spurious column headings, and this is because on the previous pages there are two objects listed next to each other. My motivation for this suggestion is that the authors could list all H II regions side-by-side, and provide an electronic table in case others wish to use these measurements in the future.

A:
We believe that makeup the paper would suffer if we remove the table from the paper.
However, we do agree that the format of table 2, as it stood in the first version, was not ideal.  

We have cut old Table 2 into 2 parts (new Table 2 + new Table 3) putting 4 objects on the first part and 3 on the last part. We guess we will have to work with the style editor to fix the problem of the table before we have a ready to publish version.

R:
5. Equation 9
Perhaps the authors would consider fitting to the number abundance of helium (y) instead of the mass fraction, when they extrapolate to the primordial value (i.e. y_p instead of Y_p). This would remove the systematic choice of having to choose a Delta Y/Delta Z_O value, and this systematic would not matter. If you still want to calculate a primordial helium mass fraction (Y_p), you could just do this after obtaining y_p.

A:
If we changed to determine y_p instead of Y_p we should obtain the same (or, at least, an extremely similar value). However we would still need to use a specific value of Delta He / Delta O. Overall this would give us the same type of uncertainty including any systematic effects. 

While equivalent the Delta Y / Delta Z_O slope is the most commonly used in the literature (in earlier papers it was Delta Y / Delta Z). This is true both, in the field of ISM abundances, as well as in the field of stellar evolution.

The last thing to consider is the effect on the choice Z_O / Z fraction. The choice of 0.55 is a very common choice, and any reasonable choice would devolve (numerically) to the same result as the determination of y_p.

R:
6. Table 6
Perhaps it would be more rigorous to quote which systematic uncertainty is the dominant one. That way, we can ascertain what is most important in pushing this fundamental measurement further. Said differently, I think it would be more informative to have a longer table that lists:
(1) H II region
(2) Y_p
(3) statistical error
(4) reddening correction error
(5) flux calibration error
(6) DeltaY/Delta Z_O error (but see Equation 9)
(7) ... another systematic
(8) ... etc.
As the authors mention in their paper, systematic errors are important, and by creating a table, the reader has a more complete idea of what systematics are the most important in the total error budget, and therefore what needs further work.

A:
We have changed the old table 6, for the new table 7, making the modifications suggested by the referee. We have also modified the 3rd paragraph of section 6 to reflect the changes to the table.


R:
7. Section 6, penultimate and final paragraphs, page 12 line 24 and line 29
This is a somewhat ambiguous statement. When saying that this is the "Planck determination", you should make it clear that this is not the value derived from the CMB damping tail, but is rather the value one gets by taking the CMB determination of Omega_B,0 h^2, combined with the Standard Model and a calculation of Big Bang Nucleosynthesis.

A: We have rewritten the last phrase of the penultimate paragraph of section 6 to be more explicit about the work done by the Planck Collaboration.

Minor comments:

R:
1. Introduction, paragraph 1, page 1 line 43-44
"such as mass-luminosity or ratio"
This text is confusing, and should be updated. I think the authors are either missing text between "or" and "ratio", or perhaps "or ratio" should be replaced by "relation".

A: 
Done

R:
2. Introduction, paragraph 1, page 1 line 45
"moreover, the chemical models, allow"
This text is also confusing. I'm not sure if "the chemical models" allow us to study the chemical enrichment, or if it just the measurements themselves that allow us to study the chemical enrichment of the Universe. Perhaps the authors mean to rephrase this as "moreover, H II region emission line abundances measured at a range of redshifts allow us to study the chemical enrichment of the Universe." But, even this, is not quite true. So, perhaps the authors should clarify this.

A:
The statement was a bit confussing, also it was a bit of a long shot. We have removed it, and re-ordered the whole sentence.

R:
3. Introduction, paragraph 5, page 2 line 31
"having a precise measurement"
It's quite easy to get a precise measurement, but the difficulty is getting an accurate measurement. I think the authors might want to rephrase this as:
"having an accurate measurement"

A:
Done

R:
4. Observations, paragraph 1, page 2 line 58
"very high spectral resolution"
perhaps state what the resolution typically is, or refrain from saying "very high", since some may consider very high to be R~100,000, or higher!

A: we have removed the over optimistic "very high" statement, it now reads "a spectral resolution of ~ 1500"

R:
5. Figure 2
Might it be useful to show the ABC region boundaries on the spectroscopy panel, too? Also, in the caption, the standard is usually to put the element and ionization ratio preceding the wavelength, and for a doublet it can be shorted to: "[N II] \lambda\lambda 6548, 6583"

A:
Done

R:
6. Section 4.1, paragraph 2 (page 8 line 53-55)
I think you can remove "all moderately high temperatures", as it is a relative concept. This may not be "moderately high" to another reader. For example, you could clarify that this is moderately high, or even typical, for an H II region of this metallicity.

A: We have included a sentence indicating what we mean for moderately high metallicities.

R:
7. Section 4.1, paragraph 3 (page 8 line 5)
"order of magnitude larger than the true density"
Since we don't know the "true" density, perhaps "expected" is a better choice of words:
"order of magnitude larger than the expected density"

A:
Done

R:
8. Section 6, page 11 line 51 and line 59
I think the authors can remove the final sentence about Izotov in both of these paragraphs. I don't think this "conflict" affects their paper.

A:Done

R:
9. The authors cite the works by Mangano et al. (2005, 2011) when discussing laboratory measurements of the neutron lifetime and number of neutrino species. I don't think these references are relevant here; the 2005 paper is an estimate of the conversion of Nnu to Neff due to neutrino decoupling, while the 2011 work is based on astrophysical limits (of which there are many). For the neutron lifetime, you may wish to cite the more recent result, by Pattie et al., and regarding the number of neutrino species, the authors should cite something that measures the decay width of the Z boson based on a laboratory experiment. Here are some more suitable references:

https://ui.adsabs.harvard.edu/abs/2018Sci...360..627P/abstract
https://ui.adsabs.harvard.edu/abs/2006PhR...427..257A/abstract

A: Done

-------

Typographical comments:

R:
1. Abstract:
"for a value Delta Y/Delta O"
This should be Delta Z_O, to keep consistency with the rest of the paper.

A:
Done

R:
2. Introduction (paragraph 4), page 2, line 15
"primordial chemical composition (...); furthermore, these..."
the semi-colon should be replaced with a full stop:
"primordial chemical composition (...). Furthermore, these..."

A:
Done

R:
3. Introduction (paragraph 4), page 2, line 18
"...close to the primordial and..."
missing the word "value":
"...close to the primordial value and..."

A:
Done

R:
4. Observations, page 2 line 48
"We also corrected by effects"
remove spurious "by":
"We also corrected effects"

A:
Done

R:
5. Figures 1, 2, 3 caption:
"the slit was presented by the"
Perhaps make the change:
"the slit is indicated by the"

A:
Done

R:
6. Section 4.1, paragraph 2 (page 8 line 42 and 45)
There's only one temperature, and one zone (even though there are multiple measurements of the temperature in this zone), so I think these should both be singular:
"temperature" and "zone".

A:
Done

R:
7. Section 6, paragraph 1, page 10 line 60
"However Z/X it is ..."
you should remove the "it" so it reads:
"However, Z/X is ..."

A:
Done

___________________________________________________________________________


==> referee.tex <==
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 

MAYO 24

Comments to the Author
I want to thank the authors for doing such a thorough job on their resubmission, and for returning the manuscript so promptly - I do not require to see another version of the manuscript. I've re-read through the paper and have a few final minor thoughts, but none of these affect the acceptance of their nice paper - thanks, and congratulations!

R:
y  versus  Y:
I'm not going to force this issue, but I raise it only to clarify what I discussed in my previous response, and the fact that the choice of "Delta Y / Delta Z_O" is the leading systematic uncertainty. In Table 6 the authors quote number abundances of He/H (so these do not depend on Delta Y / Delta Z_O). To mitigate this systematic, one could fit to the number abundances and derive a primordial number abundance by fitting a linear function to y versus O/H. The intercept would be y_p, which doesn't depend on the above-mentioned systematic. If you want to report Y_p, you could convert y_p into Y_p, and so you could eliminate one of your dominant systematics - I think!

A: 
As We understand this touches 2 different points: 
1st the choice of using y or Y 
--- both should give the same result for each object, and doing it by mass is much more common.
2nd looking for a fit using our data instead of the fit  we used in previous works.
--- any fit will have some uncertainty, but we have only a handful of points and they have a very large dispersion and not a wide enough baseline (in O/H) to provide us with better error bars.  

R:
Figure 2, spectroscopy inset:
In my comments on the previous version of the manuscript, I suggested putting 4 horizontal red lines on the spectroscopy (bottom right) panel. The authors mentioned that this was "Done", but the figure wasn't changed. While the figure doesn't need to be changed, I thought I would raise this, just in case the authors have an updated version of the figure that wasn't included in the submission.

A:
We have updated the figure.

R:
Section 6, paragraph starting with "In Table 7, we show...":
There is a typo in the text: "fist" --> "first"

A: 
Done

R:
Section 6, paragraph starting with "In Figure 4, we show...":
There is a typo in the text: "mater" --> "matter"

A:
Done

R:
Table 8 and Conclusions:
The authors mention "Delta Y / Delta O" in the caption of Table 8 and in the conclusions, and they may wish to correct this to read "Delta Y / Delta Z_O", to maintain consistency throughout the paper.

A: Done

R:
Conclusions, paragraph 3:
The references have not been updated in this paragraph.

A:
Done



% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 


MAYO 12

Reviewer's Comments:

R:
Comments to the Author
The authors present a nice paper about several H II regions in three nearby metal-poor galaxies. The main goal of the paper is to measure the chemical abundances and provide a new determination of the primordial helium abundance. The paper contains new high quality data, and I am happy to accept the manuscript for publication after the authors address a few comments that I have listed below.

-------

Main comments:
R:
1. Throughout the paper, the authors have listed all recent helium abundance determinations from H II regions, with the exception of one paper by Hsyu et al.
https://ui.adsabs.harvard.edu/abs/2020ApJ...896...77H/abstract
For completeness, the authors should probably include this determination of Yp in their work. It doesn't affect their results, and also shows a "below CMB" value of the primordial helium abundance.

A:
Sorry it was an oversight; it should have been mentioned several times throughout the paper. We now have included the reference in the introduction, Table 8, Figure 4, as well two times in section 6.

R:
2. Section 3 paragraph 2
"fitting the flux ratios of the brightest Balmer lines as compared with the theoretical values..."
Doesn't this require a temperature? If so, how does this affect the primordial helium abundance determination? Is this uncertainty included in the systematics budget?

A:
We have added a sentence after equation 1 to indicate that the HI lines have a small dependence on temperature, and that we need to do this process iteratively before being able to deredden the observed lines.

An uncertainty on the proper temperature when fitting the Balmer lines produces a very small difference on the final values, and it is indeed included in the error budget. A 500 degree error on the temperature of the fitting of the H I lines will produce a very small difference in the line intensities, and the overall effect will be an error similar or smaller than 0.0001 on YP. (Of course the temperature dependence on the final determination propagates into other aspects of the final determination; but we believe we have also carefully considered and included them on the final budget: the overall ratio of HeI/HI emmisivities, the O abundance and Delta Y / Delta Z_O correction, the collisional excitation of the H and He lines)

R:
3. Table 2
Two comments: The authors quote a percentage error of each line intensity. Does this include the uncertainty of the flux calibration based on the standard star? Going further, is the error reported just the statistical error, or does it include other terms? It's best to mention this explicitly in the text.

A:
We now include this information on the last paragraph of section 3.

R:
4. Table 2
I wonder if this table would be better suited to a Supplementary table online? On the final page of the Table, there are three spurious column headings, and this is because on the previous pages there are two objects listed next to each other. My motivation for this suggestion is that the authors could list all H II regions side-by-side, and provide an electronic table in case others wish to use these measurements in the future.

A:
We believe that makeup the paper would suffer if we remove the table from the paper.
However, we do agree that the format of table 2, as it stood in the first version, was not ideal.  

We have cut old Table 2 into 2 parts (new Table 2 + new Table 3) putting 4 objects on the first part and 3 on the last part. We guess we will have to work with the style editor to fix the problem of the table before we have a ready to publish version.

R:
5. Equation 9
Perhaps the authors would consider fitting to the number abundance of helium (y) instead of the mass fraction, when they extrapolate to the primordial value (i.e. y_p instead of Y_p). This would remove the systematic choice of having to choose a Delta Y/Delta Z_O value, and this systematic would not matter. If you still want to calculate a primordial helium mass fraction (Y_p), you could just do this after obtaining y_p.

A:
If we changed to determine y_p instead of Y_p we should obtain the same (or, at least, an extremely similar value). However we would still need to use a specific value of Delta He / Delta O. Overall this would give us the same type of uncertainty including any systematic effects. 

While equivalent the Delta Y / Delta Z_O slope is the most commonly used in the literature (in earlier papers it was Delta Y / Delta Z). This is true both, in the field of ISM abundances, as well as in the field of stellar evolution.

The last thing to consider is the effect on the choice Z_O / Z fraction. The choice of 0.55 is a very common choice, and any reasonable choice would devolve (numerically) to the same result as the determination of y_p.

R:
6. Table 6
Perhaps it would be more rigorous to quote which systematic uncertainty is the dominant one. That way, we can ascertain what is most important in pushing this fundamental measurement further. Said differently, I think it would be more informative to have a longer table that lists:
(1) H II region
(2) Y_p
(3) statistical error
(4) reddening correction error
(5) flux calibration error
(6) DeltaY/Delta Z_O error (but see Equation 9)
(7) ... another systematic
(8) ... etc.
As the authors mention in their paper, systematic errors are important, and by creating a table, the reader has a more complete idea of what systematics are the most important in the total error budget, and therefore what needs further work.

A:
We have changed the old table 6, for the new table 7, making the modifications suggested by the referee. We have also modified the 3rd paragraph of section 6 to reflect the changes to the table.


R:
7. Section 6, penultimate and final paragraphs, page 12 line 24 and line 29
This is a somewhat ambiguous statement. When saying that this is the "Planck determination", you should make it clear that this is not the value derived from the CMB damping tail, but is rather the value one gets by taking the CMB determination of Omega_B,0 h^2, combined with the Standard Model and a calculation of Big Bang Nucleosynthesis.

A: We have rewritten the last phrase of the penultimate paragraph of section 6 to be more explicit about the work done by the Planck Collaboration.

Minor comments:

R:
1. Introduction, paragraph 1, page 1 line 43-44
"such as mass-luminosity or ratio"
This text is confusing, and should be updated. I think the authors are either missing text between "or" and "ratio", or perhaps "or ratio" should be replaced by "relation".

A: 
Done

R:
2. Introduction, paragraph 1, page 1 line 45
"moreover, the chemical models, allow"
This text is also confusing. I'm not sure if "the chemical models" allow us to study the chemical enrichment, or if it just the measurements themselves that allow us to study the chemical enrichment of the Universe. Perhaps the authors mean to rephrase this as "moreover, H II region emission line abundances measured at a range of redshifts allow us to study the chemical enrichment of the Universe." But, even this, is not quite true. So, perhaps the authors should clarify this.

A:
The statement was a bit confussing, also it was a bit of a long shot. We have removed it, and re-ordered the whole sentence.

R:
3. Introduction, paragraph 5, page 2 line 31
"having a precise measurement"
It's quite easy to get a precise measurement, but the difficulty is getting an accurate measurement. I think the authors might want to rephrase this as:
"having an accurate measurement"

A:
Done

R:
4. Observations, paragraph 1, page 2 line 58
"very high spectral resolution"
perhaps state what the resolution typically is, or refrain from saying "very high", since some may consider very high to be R~100,000, or higher!

A: we have removed the over optimistic "very high" statement, it now reads "a spectral resolution of ~ 1500"

R:
5. Figure 2
Might it be useful to show the ABC region boundaries on the spectroscopy panel, too? Also, in the caption, the standard is usually to put the element and ionization ratio preceding the wavelength, and for a doublet it can be shorted to: "[N II] \lambda\lambda 6548, 6583"

A:
Done

R:
6. Section 4.1, paragraph 2 (page 8 line 53-55)
I think you can remove "all moderately high temperatures", as it is a relative concept. This may not be "moderately high" to another reader. For example, you could clarify that this is moderately high, or even typical, for an H II region of this metallicity.

A: We have included a sentence indicating what we mean for moderately high metallicities.

R:
7. Section 4.1, paragraph 3 (page 8 line 5)
"order of magnitude larger than the true density"
Since we don't know the "true" density, perhaps "expected" is a better choice of words:
"order of magnitude larger than the expected density"

A:
Done

R:
8. Section 6, page 11 line 51 and line 59
I think the authors can remove the final sentence about Izotov in both of these paragraphs. I don't think this "conflict" affects their paper.

A:Done

R:
9. The authors cite the works by Mangano et al. (2005, 2011) when discussing laboratory measurements of the neutron lifetime and number of neutrino species. I don't think these references are relevant here; the 2005 paper is an estimate of the conversion of Nnu to Neff due to neutrino decoupling, while the 2011 work is based on astrophysical limits (of which there are many). For the neutron lifetime, you may wish to cite the more recent result, by Pattie et al., and regarding the number of neutrino species, the authors should cite something that measures the decay width of the Z boson based on a laboratory experiment. Here are some more suitable references:

https://ui.adsabs.harvard.edu/abs/2018Sci...360..627P/abstract
https://ui.adsabs.harvard.edu/abs/2006PhR...427..257A/abstract

A: Done

-------

Typographical comments:

R:
1. Abstract:
"for a value Delta Y/Delta O"
This should be Delta Z_O, to keep consistency with the rest of the paper.

A:
Done

R:
2. Introduction (paragraph 4), page 2, line 15
"primordial chemical composition (...); furthermore, these..."
the semi-colon should be replaced with a full stop:
"primordial chemical composition (...). Furthermore, these..."

A:
Done

R:
3. Introduction (paragraph 4), page 2, line 18
"...close to the primordial and..."
missing the word "value":
"...close to the primordial value and..."

A:
Done

R:
4. Observations, page 2 line 48
"We also corrected by effects"
remove spurious "by":
"We also corrected effects"

A:
Done

R:
5. Figures 1, 2, 3 caption:
"the slit was presented by the"
Perhaps make the change:
"the slit is indicated by the"

A:
Done

R:
6. Section 4.1, paragraph 2 (page 8 line 42 and 45)
There's only one temperature, and one zone (even though there are multiple measurements of the temperature in this zone), so I think these should both be singular:
"temperature" and "zone".

A:
Done

R:
7. Section 6, paragraph 1, page 10 line 60
"However Z/X it is ..."
you should remove the "it" so it reads:
"However, Z/X is ..."

A:
Done

___________________________________________________________________________

